Multi-Agent Off-Policy TD Learning: Finite-Time Analysis with Near-Optimal Sample Complexity and Communication Complexity

The finite-time convergence of off-policy TD learning has been comprehensively studied recently. However, such a type of convergence has not been well established for off-policy TD learning in the multi-agent setting, which covers broader applications and is fundamentally more challenging. This work develops two decentralized TD with correction (TDC) algorithms for multi-agent off-policy TD learning under Markovian sampling. In particular, our algorithms preserve full privacy of the actions, policies and rewards of the agents, and adopt mini-batch sampling to reduce the sampling variance and communication frequency. Under Markovian sampling and linear function approximation, we proved that the finite-time sample complexity of both algorithms for achieving an $\epsilon$-accurate solution is in the order of $\mathcal{O}(\epsilon^{-1}\ln \epsilon^{-1})$, matching the near-optimal sample complexity of centralized TD(0) and TDC. Importantly, the communication complexity of our algorithms is in the order of $\mathcal{O}(\ln \epsilon^{-1})$, which is significantly lower than the communication complexity $\mathcal{O}(\epsilon^{-1}\ln \epsilon^{-1})$ of the existing decentralized TD(0). Experiments corroborate our theoretical findings.

==> tex/experiments_Yi.tex <==
We simulate a multi-agent MDP with 5 fully decentralized agents. The shared state space contains 10 states and each agent can take 2 actions. All behavior policies are uniform policies (i.e., each agent takes all actions with equal probability), and the target policies are obtained by first perturbing the corresponding behavior policies with Gaussian noises sampled from \red{$\mathcal{N}(0, 0.05)$} and then performing a proper normalization. The entries of the transition kernel and the reward functions are independently generated from the uniform distribution on $[0,1]$ (with proper normalization for the transition kernel).\red{ The entries of the features are independently generated from the standard Gaussian distribution with proper normalization. }The discount factor is set to $\gamma=0.95$. We consider two network topologies: fully connected network \red{(The communication matrix $V$ has diagonal entries 0.9 and off-diagonal entries 0.025.)} and ring network \red{($V$ has diagonal entries 0.8, entries 0.1 for any pair of neighboring agents, and other entries 0)}. 

We compare the sample complexities and communication complexities (for synchronizing model parameters) of the following algorithms: decentralized TD(0) \cite{sun2020finite}, decentralized TDC with mini-batch sizes $N=10,20,50,100$,respectively. We set learning rate $\alpha=0.01$ for decentralized TD(0) and $\alpha=0.01*N$, $\beta=10^{-4}*N$ for decentralized TDC. 
In all experiments, each algorithm is tested on the same 100 MDP trajectories, each of which consists of 10k Markovian samples. 

\subsection{Exact Global Importance Sampling}
We first test all the decentralized TD algorithms with a fully connected network, whose communication matrix $V$ has diagonal entries $0.9$ and off-diagonal entries $0.025$. The convergence error $\|\overline{\theta}_t-\theta^*\|^2$ v.s. the sample complexity and communication complexity are shown in Figure \ref{fig1}.

Our second experiment is conducted in the same way as the first experiment, except that the loop network is used where each agent connects to itself and its two neighboring agents with weights 0.8 and 0.1 respectively. The result plots are shown in Figures \ref{fig3}\&\ref{fig4}, corresponding to Figures \ref{fig1}\&\ref{fig2} of the first experiment respectively. 


\subsection{Inexact Global Importance Sampling}
Furthermore, we compare \Cref{alg: 1} (exact $\rho$) and \Cref{alg: 2} with inexact $\rho$ obtained via $L=1,2,3,4$ communications. We set $\alpha=??$, $\beta=??$ and use ?? iterations. We also add the decentralized TD(0) with exact $\rho$, $\alpha=0.01$ and batchsize 1 as a baseline. The result plots with the same metric above are shown in Figure \ref{fig2}. ??......
